The Quasar Outflow Contribution to AGN Feedback: VLT Measurements of SDSS J0318-0600

We present high spectral resolution VLT observations of the BAL quasar SDSS J0318-0600. This high quality data set allows us to extract accurate ionic column densities and determine an electron number density of n_e=10^3.3 +/- 0.2 cm^-3 for the main outflow absorption component. The heavily reddened spectrum of SDSS J0318-0600 requires purely silicate dust with a reddening curve characteristic of predominately large grains, from which we estimate the bolometric luminosity. We carry out photoionization modeling to determine the total column density, ionization parameter and distance of the gas and find that the photionization models suggest abundances greater than solar. Due to the uncertainty in the location of the dust extinction, we arrive at two viable distances for the main ouflow component from the central source, 6 and 18 kpc, where we consider the 6 kpc location as somewhat more physically plausable. Assuming the canonical global covering of 20% for the outflow and a distance of 6 kpc, our analysis yields a mass flux of 120 M_sun yr^-1 and a kinetic luminosity that is ~0.1% of the bolometric luminosity of the object. Should the dust be part of the outflow, then these values are ~4x larger. The large mass flux and kinetic luminosity make this outflow a significant contributor to AGN feedback processes.

==> Table1.tex <==
%\begin{center}
\begin{deluxetable}{lcccccc}
\tablewidth{0.7\textwidth}
\tablecolumns{7}
\footnotesize
\tablecaption{VLT Observations of QSO J0318$-$0600}

\tablehead{
\colhead{Date} &
\colhead{Time$^a$} &
\colhead{JD$^b$} &
\colhead{Airmass} &
\colhead{Seeing} \\
}

\startdata
30 Sep 2006 & 04:35:01 & 54008.19092 & 1.41 & 1.08 \\
01 Oct 2006 & 03:51:30 & 54009.25268 & 1.12 & 1.07 \\
01 Oct 2006 & 06:53:51 & 54009.28740 & 1.06 & 0.97 \\
15 Oct 2006 & 05:55:23 & 54023.24679 & 1.06 & 1.00 \\
19 Oct 2006 & 05:34:22 & 54027.23220 & 1.07 & 0.82 \\
20 Oct 2006 & 06:49:21 & 54028.28427 & 1.07 & 0.71 \\
22 Oct 2006 & 04:45:58 & 54030.20063 & 1.10 & 0.66 \\
22 Oct 2006 & 05:38:28 & 54030.23505 & 1.06 & 0.55 \\
\enddata
\normalsize
\tablenotetext{a}{Exposure time for each observation was 2800s}
\tablenotetext{b}{Julian Date presented in days +2400000}
\label{obs}
\end{deluxetable}
%\end{center}
\thispagestyle{empty}


==> discussion.tex <==
\section{Discussion}


\begin{deluxetable}{lcccccc}
\tablecolumns{7}
\tabletypesize{\footnotesize}
\tablecaption{Properties of Measured Outflows to Date}
\tablehead{
\colhead{Object} &
\colhead{$R$$^a$} &
\colhead{log $N_H$} &
\colhead{log U$_H$} &
\colhead{log $\dot{E_k}$} &
\colhead{$\dot{M}$} &
\colhead{Reference$^b$} \\

\colhead{\small{}} &
\colhead{\small{(kpc)}} &
\colhead{\small{(cm$^{-2}$)}} &
\colhead{\small{}} &
\colhead{\small{(ergs s$^{-1}$)}} &
\colhead{\small{($M_\sun$ yr$^{-1}$)}} &
\colhead{\small{}} \\
}
%\footnotesize
\startdata
QSO 0059-2735   & 0.001 - 0.05 & $\gtrsim$21.5$^c$ & $-$0.7      & $\gtrsim$41.1 - 42.8&$\gtrsim$0.2& 1 \\
3C~191          & 28           & 20.3         & $-$2.8           & 44.0         & 310        & 2 \\
QSO 1044+3656   & 0.1 - 2.1    & 20.0 - 22.0  & $-$1.0 - $-$6.0  & 44.5 - 45.4  & 74 - 530   & 3 \\
FIRST 1214+2803 & 0.001 - 0.03 & 21.4 - 22.2  & $-$2.0 - $-$0.7  & 41.6 - 43.8  & 0.3 - 55   & 4 \\
FIRST 0840+3633 & 0.001        & $\sim$21.3   & $<$$-$1.8        & $>$41.9      & $>$0.3     & 5 \\
FIRST 0840+3633$^d$ & 0.23     & $-$          & $-$              & $-$          & $-$        & 5 \\
QSO 2359-1241   & 3            & 20.6         & $-$2.4           & 43.7         & 93         & 6 \\
SDSS J0838+2955 & 3.3          & 20.8         & $-$1.9           & 45.7         & 590        & 7 \\
SDSS J0318-0600 & 6 or 17      & 19.9 or 20.0 & $-$3.1 or $-$2.7 & 44.8 or 45.4 & 120 or 450 & 8 \\
\enddata
\tablenotetext{a}{For relative accuracies, see Section 1.}
\tablenotetext{b}{1-Wampler et al. (1995), 2-Hamann et al. (2001), 3-de Kool et al. (2001),
4-de Kool et al. (2002a), 5-de Kool et al. (2002b), 6-Korista et al. (2008),
7-Moe et al. (2009), 8-This Work}
\tablenotetext{c}{Based on Table 5 in Wampler et al. (1995)}
\tablenotetext{d}{Distance derived from \feii\ fluorescence and no photoionization modeling
was performed for this object}
\normalsize
\label{summary}
\end{deluxetable}

In this section we compare the results from this object to other
outflows found in the literature; discuss the location of the dust in
SDSS~J0318$-$0600, which is a major cause for uncertainty in the
derived mass flux and kinetic luminosity; elaborate on the
relationship between the dynamical time scale of the outflow and the
duty cycle of the quasar; and conclude by describing the possible role
of these outflows in AGN feedback phenomena

In Table \ref{summary} we compare all the analyses in the literature
that can be used to obtain mass flux and kinetic luminosity for
outflows in individual quasars. We also note that with the exception
of SDSS~J0318$-$0600, every absorber shows evidence for inhomogeneous
line of sight (LOS) covering. For outflow absorption, we refer to
homogeneity as the spatial distribution of gas across our line of
sight to the quasar (see section 3.2), where a homogeneous flow would
uniformly cover the background emission source (LOS covering factor of
1). Initially, this may be attributed is to the large
distance of the absorber, however, the outflow in
3C~191 shows evidence of inhomogeneous covering at a greater distance
than we find component {\bf i} of SDSS~J0318$-$0600.

SDSS~J0318-0600 is also the most heavily reddened in the sample, which
leaves us with the question of the location of the obscuring
dust. Based on the value from \citet{1998ApJ...500..525S}, we know
that the Milky Way Galactic reddening is minimal, and thus the
reddening is intrinsic to the quasar.  There exist three possible
locations of the dust with respect to the absorber: interior,
dispersed within, and exterior. The two locations for the dust we
consider here due to their potential impact on the modeling of the
outflow are that the dust is interior to the absorber or the dust is
associated with the absorber. If the dust is interior to the absorber,
a plausible source of dust would be the edge of the putative obscuring
torus of the AGN unified model \citep{1985ApJ...297..621A}. This is
supported by the object discussed by Aoki et al. (2009, in
preperation) and furthermore would provide the rare sight line needed
to match the frequency of detections for low ionization BAL outflows
that show iron absorption (FeLoBAL), as discussed in section 5.1. By
contrast, galactic wind imaging in nearby galaxies shows that dust
co-exists inside the winds and may be associated with the outflows
\citep[e.g., M82,][]{1994ApJ...433..645I}. \citet{2002ApJ...567L.107E}
proposed the possibility of grains forming within AGN outflows, as
conditions allowed. We note though that if the outflowing gas contains
the observed dust, the amount of dust depletion must be substantially
smaller than in the ISM or SMC in order to produce the observe ionic
column densities. Therefore, while we cannot strongly exclude the
possibility of a dusty outflow, locating the dust at the edge of the
putative torus is physically more plausible and explains several
observed features in the FeLoBAL population: the heavy reddening of 
FeLoBALs, the low reddening experienced by \civ\ BAL quasar; and the 
higher prevalence of high ionization BALSQSOs compared with FeLoBALs.

The dynamical time for component $\bf i$ of the outflow is
$t_d=R/v\approx10^6$ yr (assuming $R=6$ kpc). Therefore, if we are
seeing a representative stage of the outflow, over its $\sim$10$^8$ yr
duty cycle \citep []{2005ApJ...625L..71H} the quasar must eject
roughly hundred times more mass than is seen in component $\bf i$. 
Obvious candidates for more ejected mass are the other 10
components of the outflow. However, Bautista et al. (2009, in prep)
show that these components collectively do not contribute
appreciably to the total mass output for SDSS~J0318$-$0600. Earlier 
episodes of mass ejection may not be detectable in
absorption. Let us assume that component $\bf i$ is continuing at
a constant velocity and no longer entraining any significant mass.
Within $10^7$ yr, its distance will increase by a factor of ten and 
therefore its optical depth will drop by a factor of a hundred, making 
it undetectable in absorption. To complete the picture we note that in 
addition to the FeLoBAL system, SDSS~J0318$-$0600 has a high ionization 
BAL at $\sim$27000 km s$^{-1}$. This outflow component is probably 
much closer and therefore represent a very young mass ejection episode 
that in time may evolve to something resembling component $\bf i$. 
Similar situation exist in other objects 
\citep[e.g. SDSS~J0838+2955;][]{2009ApJ...706..525M}.

Given these caveats the kinetic luminosity, such as the one we have
measured in \\
SDSS~J0318$-$0600, provides
$\sim$(0.1-0.6)$\Omega_{0.2}$\% of the bolometric luminosity as
feedback. We note that the measured mass of component $\bf i$
represents only the cold phase (T=10$^4$ K) of the outflow. The hot
phase of the gas (or X-ray, T=10$^6$ K) has been shown in Seyfert
galaxies \citep[e.g., NGC 3783;][]{2003ApJ...599..933N} to contribute
up to 50$\times$ more column density than the cold phase, therefore it
is possible that the gas in the hot phase of the outflow in
SDSS~J0318$-$0600 could contribute significantly to the mass flux and
kinetic luminosity. For comparison, AGN feedback models of galaxy
growth and evolution require a mechanical energy input of roughly 5\%
of the bolometric luminosity of the quasar. For example,
\citet{2005Natur.433..604D} use this ratio to recreate the observed
M$_{BH}$-$\sigma$ relation and \citet{2005ApJ...630..705H} show
in their models that the same value is required to `uncover' a 
shrouded quasar after a merger. Thus, the absorption outflow we observe 
in SDSS~J0318$-$0600 can be a significant contributer for AGN feedback 
processes.

Beyond the effects of feedback on the host galaxy, if SDSS~J0318$-$0600
is representative of the type of quasars found in clusters, then we
also see that an outflow with the kinetic luminosity of
SDSS~J0318$-$0600 would contribute energy to the gas that forms the
ICM. The models of \citet{2004ApJ...608...62S} show that a 5\%
feedback ratio would suffice to heat the ICM during formation of the
cluster and provide the well known L$_x$-T relationship
\citep{1986MNRAS.222..323K,1999MNRAS.305..631A}
Also, related to clusters are X-ray cavities in the ICM, which coincide
with relativistic radio jets \citep[e.g. NGC1275 in the Perseus
cluster,][]{2006MNRAS.366..417F}. We suggest that the sub-relativistic
outflows could be related to the bubbles or perhaps are the driving
mechanisms for bubble inflation. This follows as the inflation of
a bubble is a simpler process provided a wide angle wind 
\citep{2007ApJ...656L...5S}. \citet{2006ApJ...652..216R} shows that the 
power needed to inflate these bubbles is $\sim$10$^{45}$ ergs s$^{-1}$, 
which is similar to the kinetic luminosity we measure in SDSS~J0318$-$0600 
of $\sim$1-3$\times$10$^{45}$ ergs s$^{-1}$. These similarities in fraction 
of the bolometric luminosity and power output suggest that quasar outflows 
play significant roles in influencing their host galaxy and neighborhoods
through feedback.


==> measurements.tex <==
\section{Detection \& Measurements}

The spectrum of SDSS~J0318$-$0600 contains a plethora of absorption 
features available for potential diagnostics. In Figure \ref{f1}, we 
show a sample of the VLT spectrum with line identifications, and 
present the full spectrum with identifications in our online figure. 
These identifications come from matching the \mgii\ doublet lines 
and plotting location identifiers for other ionic lines. We also 
provide an online table for all identified lines, their wavelengths, 
oscillator strengths and references. We show in Figure 1 a portion of
the full online figure that contains readily visible lines from both 
the ground as well as excited levels of \feii\ (lower energy levels 
up to 1873 cm$^{-1}$).

\begin{figure}[!h]
  \centering \includegraphics[angle=90,width=0.9\textwidth]
  {Fig1.eps}\\ 
  \caption[] 
  {\footnotesize
Portion of the VLT spectrum showing the \feii\ UV 38 multiplet 
in SDSS~J0318$-$0600 (the full spectrum can be found online). Line 
identifications are indicated by vertical blue lines for the expected 
position of component $\bf i$, based on the redshift z=1.9257. 
The redshift of the quasar is in black located at the top right. The 
log($gf$) values of the identified transitions are shown above the 
spectrum, where $g$ is the statistical weight and $f$ is the oscillator 
strength. The size of the vertical blue line provides the value, which 
can be read from the y-axis scale at the top right. Each identifier 
lists the ion, wavelength, and lower energy level (in 1000s of 
cm$^{-1}$). The spectrum error is plotted in solid black below the 
spectrum ($\approx$0.05 in normalized flux).}
  \label{f1}
\end{figure}

\subsection{Identification of Kinematic Components}

We identify each of the individual kinematic absorption components in 
the spectrum using the \alii\ $\lambda$1671 absorption line profile, 
which is a singlet transition with no nearby strong absorption features. 
In Figure \ref{f2}, we show that there are approximately 11 separate 
kinematic components (labeled $\bf a-k$), with component $\bf e$ 
clearly a blend of multiple inseparable components. Using \alii\ 
as a template for the absorbers we search other ionic species for each 
of the 11 components.

Next, we identify the broad, strong $\bf i$ component in as many  
lines as possible and select unblended troughs from which we are 
able to measure ionic column densities. Figure \ref{f1} shows the 
UV 38 \feii\ multiplet, which exhibits several absorption features 
from component $\bf i$. We note that the absorption feature at 
$\sim$4727 \AA\ is the $\bf k$ component of the \feii\ $\lambda$1608 
resonance line. While this identification scheme is sufficient to 
locate the majority of the lines that show an $\bf i$ component, we 
also use the \alii\ as a template (see $\S$3.3), to search for the 
other 10 components in the \feii\ UV 1, 2 \& 3 multiplet absorption 
complexes. 

%\clearpage
\noindent
\begin{rotate}
\begin{figure}
 \noindent
 \hspace{-2.5in}
 \begin{minipage}[t]{4.0cm}%\linewidth} A minipage that covers half the page
  \vspace{-2.5cm}
  \includegraphics[width=13.5cm,height=17.5cm]{Fig2a.eps}
 \end{minipage}
 \hspace{3.2in} % To get a little bit of space between the figures
 \begin{minipage}[t]{4.0cm}%\linewidth}
  \vspace{-2.5cm}
  \includegraphics[width=13.5cm,height=17.5cm]{Fig2b.eps}
 \end{minipage}
\caption{\scriptsize The main outflow troughs in SDSS~J0318$-$0600, 
ordered by wavelength. We identify the 11 kinematic components found in
\alii\ from high to low velocities, which we label $\bf a$ through $\bf k$.
In the plots of \feii\ $\lambda$2383, $\lambda$2396, and $\lambda$2600 there
are several contaminate lines present due to the telluric A and B bands as 
well as blending from other \feii\ troughs (identified in online figure). 
Each doublet also shows blending between components (e.g. \civ, \mgii).}
\label{f2}
\end{figure}
\end{rotate}

%\clearpage
\input{Table2}
\clearpage

The \feii\ multiplets UV 1, 2 \& 3 are the best candidates to identify \feii\
lines from the other 10 components to measure, because they contain the 
\feii\ transitions with the strongest oscillator strengths. However, this 
task proves to be non-trivial in SDSS~J0318-0600. Identifying measurable 
lines from a saturated and heavily blended region (see Figure \ref{f2}) 
is difficult, especially when considering the large number of strong 
resonance and excited state lines. Our strategy is to make what line 
identifications for all 11 components that we can using our \alii\ 
template and search for other lines where the blending is not so 
prevalent. We provide the full list of detected ions, transition 
wavelengths, their oscillator strengths and lower level energies in the 
online table. 

%One detection example, is the \niII\ $\lambda$2217 excited 
%state line shown in Figure \ref{f2}, where we can identify components 
%$\bf b$, $\bf d$, $\bf g$, $\bf h$, and $\bf k$, beyond the
%identification of the strong component $\bf i$. 

We find that for the lowest and highest velocity components 
($\bf k$ and $\bf a$), enough measurements or limit determinations are 
available that we can effectively determine the electron density ($n_H$), 
the ionization parameter (U$_H$), and the total hydrogen column density 
($N_H$, see $\S$4). Unfortunately, blending prevents us from identifying 
enough measurable troughs for components $\bf b-h$ for proper analysis. 
We opt for the limiting case by taking the sum of these latter systems 
(see $\S$3.2).

\subsection{Column Density Determinations}

With a list of measurable absorption troughs, we 
extract ionic column densities. We begin the process by measuring 
lines from the strongest component, ($\bf i$), where we employ three
primary methods for determining the column densities. We describe 
three additional methods for column density determination that are less
reliable in section 3.3. We provide the measured values of ionic 
column densities as well as the method applied in Table~\ref{compi}.

Our first method of measuring column densities is to model a set of 
observed \feii\ resonance lines (e.g., Figure \ref{f3}) using an
inhomogenous absorption model, where we approximate the gas 
distribution across our line of sight to the background source with a 
power law \citep[see][especially Fig. 4, for a full description]
{2002ApJ...580...54D,2008ApJ...681..954A}. The optical depth at a 
given velocity within the outflow is described by: 
\begin{equation}
\tau_v(x) = \tau_{max}(v) x^a ,
\end{equation}
where $x$ is the spatial dimension in the plane of the sky 
\citep[simplified to one dimension with no loss of generality, see][]
{2005ApJ...620..665A}, $a$ is the power law distribution index, and
$\tau_{max}(v)$ is the highest value of $\tau$ at a given velocity. 
We simultaneously solve for 
both $\tau$$_{max}$ and $a$ for each velocity resolution element of 
the resonance \feii\ lines and apply this distribution ($a$) to the 
excited \feii\ lines. We then apply the same distribution dictated by 
the \feii\ lines to all ions because this is the simplest assumption 
that imposes the strongest constraints.

We convert the modeled $\tau$$_v$ to column density via 
\citep{1991ApJ...379..245S}:
\begin{equation}
N(v) = 3.8 \times 10^{14} \frac{1}{f\lambda} \tau_v~(cm^{-2} km^{-1} s),
\end{equation}
where $\lambda$ is the wavelength of the line in \AA, $f$ is the oscillator
strength, and $\tau$$_v$ is the optical depth in velocity space in 
km~s$^{-1}$, which is integrated over the spatial dimension $x$. Using 
Equation 2, we compute the column density for each 
velocity element and integrate over the range in velocity, which we justify 
later in this section. In Table~\ref{compi}, we 
quote the power law estimation of the column densities (when available) 
as this is the most accurate and most plausibly physical explanation of 
non-black saturated absorption at large distances 
\citep{2008ApJ...681..954A,2002ApJ...580...54D}. In Table~\ref{compi} and 
throughout this paper, we will refer to this as method 1.

Method 2 is to model the \feii\ resonance lines with a velocity 
dependent line of sight (LOS) covering factor. The LOS covering factor 
in this case is a geometric step-function distribution \citep[see 
Figure 4 in][]{2008ApJ...681..954A}. In other words, a fraction of the 
extended source is completely obscured by the outflow, while the rest 
of the source is uncovered. We assume that each radial velocity element 
has an independent LOS covering factor, which we again determine using 
the \feii\ resonance lines. We solve a fitting equation for $\tau$$_v$ 
\citep{2005ApJ...620..665A}:
\begin{equation}
I(v) = 1 - C(v) + C(v) e^{-\tau(v)},
\end{equation}
where $I$ is the normalized intensity within the trough and $C(v)$
is the velocity dependent LOS covering factor. First, we solve Equation
(3) for $C(v)$ and $\tau$$(v)$ using at least two resonance lines from 
\feii. We then calculate the velocity dependent column density using
$\tau$$(v)$ in Equation (2) and multiply the column density at each
velocity by $C(v)$
to obtain the average column density across the line of sight. Finally,
we compute the total ionic column density by integrating across the 
velocity range of the trough. This method is comparable in accuracy 
to method 1 \citep{2008ApJ...681..954A}, and the column density 
results are approximately the same as found by method 1.

The last of the three methods, method 3, is simply the apparent optical 
depth method \citep[AOD,][]{1991ApJ...379..245S}. 
This method assumes that all photons traveling to the observer pass
through the same amount of gas at a given velocity, which gives the
equation for normalized intensity: $I(v)$=$e$$^{-\tau(v)}$. We again 
convert to column density via Equation (2) and integrate to find the 
total ionic column density. This method does not account for partial LOS
covering and saturation effects in line centers, which can underestimate 
column densities by up to an order of magnitude. However, we find that 
for SDSS~J0318-066, in most cases a LOS covering factor of 1 (i.e. the 
AOD approximation) yields similar N$_{ion}$ values as those derived by 
the power law or partial covering method, a point 
we will discuss later in this section.

For the upcoming photoionization modeling, we adopt the ionic column 
densities as determined by method 1 (power law method) with some 
exceptions to this due to line blending that are noted in Table~\ref{compi}. 
We now present our analysis for the individual components.

\subsubsection{Measurements of Component $\bf i$}

We begin our column density determination by fitting the \feii\
resonance lines from the strongest component, ($\bf i$). In Figure 
\ref{f3}, we show the fits for three \feii\ resonance lines using 
the power law method. We select these particular line transitions 
because they provide us with a range of oscillator strengths and 
are free of blending or telluric contamination. Using these lines, 
we derive velocity dependent column densities that we integrate 
for the total ionic column density. 

Unfortunately, all strong \feii\ lines from the lower energy level 
385 cm$^{-1}$ are heavily blended in the UV 1, 2 or 3 multiplets with 
lines from both the resonance and other excited lines (e.g., \feii*
$\lambda$2396, shown in Figure \ref{f2}), which renders column 
density measurements based on these transitions to have large 
systematic errors. However, we find relatively strong lines outside 
of the UV 1, 2 or 3 multiplets for the 385 cm$^{-1}$ energy state
that are useful such as the \feii\ line $\lambda$1622 from the UV~38
multiplet. We also find two weaker lines from this energy state at 
$\lambda$1619 and $\lambda$2281 that are unblended. The oscillator 
strength values for these three lines are taken from Fuhr \& Wiese 
(2006). Of the three lines, both the $\lambda$1618 and $\lambda$1622 
are reported to have accurate oscillator strengths (rated as 
``A''\footnote{Accuracies of``A'', ``B'' and ``C'' are applied to
oscillator strengths with uncertainties less than 3\%, 10\% and 25\%,
respectively, according to the NIST Atomic Spectra Database} by Fuhr 
\& Wiese), while the weaker $\lambda$2281 has a 
reasonably reliable oscillator strength (rated ``B''). 
However, we find that using the oscillator strengths reported by Fuhr 
\& Wiese to be problematic. While the two weaker lines are well fit 
with these oscillator strengths, the trough depths relative to 
$\lambda$1622 are unphysical. For example, scaling the $\lambda$1619 
trough in apparent optical depth by the ratio of oscillator strengths 
($\sim$1.8) should be equal to the apparent optical depth in 
$\lambda$1622 (or larger in the case of partial covering), however 
the scaled optical depth of $\lambda$1619 is significantly smaller
than that of the $\lambda$1622 trough. This means that at least one 
of the oscillator strengths could be less reliable than previously 
believed. Because of this issue, we quote an ionic column density for 
the 385 cm$^{-1}$ energy level that is the mean of the fit to the 
$\lambda$1622 line alone and the fit to the two weaker lines with an 
uncertainty equal to the range in column density.

\begin{figure}[!h]
  \centering \includegraphics[angle=90,width=0.7\textwidth]
  {Fig3.eps}\\
  \caption[]
  {\footnotesize
The line fits for the three uncontaminated \feii\ resonance lines based
on the power law method. The data are presented in 7 km s$^{-1}$ bins
with a solid line (statistical observational error bars for these data
are also shown), while the model fit is shown by a dotted line.
Each line is color coordinated with the wavelength located at the lower
left of the plot.}
  \label{f3}
\end{figure}

\begin{figure}[!h]
  \centering \includegraphics[angle=90,width=0.7\textwidth]
  {Fig4.eps}\\
  \caption[]
  {\footnotesize
The power law model fits for four lines of metastable
\feii\ (E$_{low}$=1873 cm$^{-1}$), we use the exponential $a$
parameter calculated from resonance \feii. Similar to Figure 3.}
  \label{f5}
\end{figure}

The other excited state lines from \feii\ (e.g., arising from 668, 
863, and 977 cm$^{-1}$) are also subject to heavy blending in the 
multiplets, but unlike the resonance and 385 excited state lines 
there is not sufficient column density to provide deep troughs with 
high signal-to-noise for the weaker lines. Thus, the column density 
measurements from these energy levels are significantly more 
uncertain. The exceptions to this are lines from the lower energy 
level state 1873~cm$^{-1}$ ($^4$F) and 7955~cm$^{-1}$ ($^4$D).

We find 5 separate absorption troughs of \feii\ arising from the 
level at 1873~cm$^{-1}$, which are shown in Figure \ref{f5}. We 
successfully fit these using the oscillator strengths from 
\citet{1995all..book.....K} to determine the column density for this 
level. However, the compilation of recommended oscillator strengths of 
\feii\ from Fuhr \& Wiese (2006) yields values lower by $\sim 0.3$~dex 
for two of the transitions, $\lambda$1637.4 and $\lambda$1702.0. For 
these transitions the recommended values are rated ``C'', while no 
oscillator strengths are given for the other two observed transitions. 
In addition to the difference in the absolute values, there is also a 
difference in the relative values, and in fact our fits to the absorption
troughs in the spectrum favors the relative values of Kurucz \& Bell (1995). 
Thus, we opt to use the relative oscillator strengths from Kurucz \& Bell 
(1995) to fit all four troughs, but the level column density derived this 
way is increased by 0.3~dex, as required by the absolute oscillator 
strengths of Fuhr \& Wiese. 

We find that the results from all three models (Power law, covering
factor, and AOD) are similar for the 
\feii\ column density measurements of component $\bf i$, which 
suggests that the LOS covering factor of the system is close to 1. 
Further evidence for a LOS covering factor$\approx$1 case is given 
in Figure \ref{f8a}, where we show that we can use the \alii\ template 
to fit the \aliii\ doublet. We scale two \alii\ templates
(one for \aliii\ $\lambda$1855 and one for \aliii\ $\lambda$1863) in 
$\tau$ space for each individual kinematic component for the blue and 
the red line of the doublet by the expected ratio of 2:1 and coadd the 
templates to generate a fit to the data. There exist only small 
deviations, and the overall fit to the doublet is good. The most 
obvious and important deviation is in the fit to the $\lambda$1863 
$\bf i$ component, which is due to some saturation in the core of the 
\alii\ template. This demonstrates that AOD is an adequate 
approximation and the LOS covering factor for all components is 
approximately 1.0. This same procedure gives similar results when 
applied to the \mgii\ doublet as well. 

\begin{figure}[!h]
  \centering \includegraphics[angle=90,width=0.7\textwidth]
  {Fig5.eps}\\
  \caption[]
  {\footnotesize
The \aliii\ doublet plotted in velocity space with respect to the blue
member of the doublet. The blue and red
tickmarks and letters indicate the component positions of the \aliii\
doublet members, \aliii\ $\lambda$$\lambda$1855,1863 respectively.
The dotted blue and red lines are the individual \alii\ template
fits for each member of the doublet (corresponding to the blue and
red tickmarks). Each individual component is scaled in $\tau$ and the
resulting templates match the expected doublet ratio of 2:1 for each
of the components. We coadd, in $\tau$ space, the two \alii\ templates 
and present the resulting fit in green. The fit agrees with the data
with the exception of the $\lambda$1863 component $\bf i$, which is
likely due to saturation in the $\lambda$1855 counterpart.}
  \label{f8a}
\end{figure}

\begin{figure}[!h]
  \centering \includegraphics[angle=0,height=0.7\textwidth,width=0.6\textwidth]
  {Fig6.eps}\\
  \caption[]
  {\footnotesize
Component $\bf i$ column density ratios of \feii*/\feii\ and 
\siII*/\siII, top and bottom respectively, in velocity space. 
Within the error bars the ratios are constant across the 
integration range. This indicates that the outflowing gas has 
a constant electron number density across the trough, which 
strongly suggests similar ionization conditions across the 
velocity span of this outflow component.}
  \label{f6}
\end{figure}

\subsubsection{The Physical Connection Between Material Seen in Different Troughs}

Ultimately, we want to establish the physical characteristics of
the outflow based on the column density determinations described
above.  In order to do so we use the integrated column densities as
input to photioinization models, which in turn determine the total
hydrogen column density and number density in the outflow.  This
procedure depends on two assumptions: 1) that the physical conditions
do not change as a function of velocity across a given trough. This
assumption allow for the use of integrated column densities instead of
working with each velocity resolution element separately (see Arav et
al 2007); 2) That the troughs of different ions correspond to the same
outflowing gas, which is a necessary condition for using these
measurements in the same photoionization models. Both assumptions can 
be checked using the data at hand.

The first assumption can be tested by checking the ratio measured
column densities amongst different lower levels of the same ion vary
as a function of velocity. In figure \ref{f6} we plot the ratios of
column densities between those arising from excited levels to those
from the ground state level of \feii\ and \siII. Within the
uncertainties, the ratios across the troughs are velocity independent,
showing that the electron number density is constant across the flow
(see \S~4 for elaboration).  This result gives validity to our first
assumption and justify the use of integrated column densities for
component {\bf i}. We also tested this for \niII/\niII* and
combinations between \niII, \siII\ and \feii\ resonance and excited
lines and find that the ratio is constant in all cases. This constant
ratio is also seen in the results for the outflow system in
QSO~2359$-$1241 as described by \citet{2008arXiv0807.0230K}.

In order to validate the second assumption we need to check the column
density ratio across troughs from different ions and especially
compare low and high ionization troughs. To do so we use the $\tau(v)$
profile of \siII\ $\lambda$1527 and attempt to fit the profiles of
other troughs while using a single scale factor for each line.  The
results are shown in figure \ref{f7a}. It is evident that the scaled
$\tau(v)$ profile of \siII\ $\lambda$1527 fits the troughs of \siiv,
\alii, \aliii\ troughs and \mgii\ remarkably well, lending strong
support for the assumption that we are measuring the same outflowing
gas.  For \civ, which is the highest ionization line observed, the fit
for the center of the trough is less conclusive since the trough is
highly saturated at its core.  However, we point out the the fit to
the low velocity wing (--3950 to -3850 \kms) is very good, which would
be a coincident unless the \civ\ trough can be fitted with the same
$\tau(v)$ profile of \siII\ $\lambda$1527.  In summary, the data
support the two main assumption that we need in order to use all
integrated column densities in our photoionization models.

To demonstrate the tie between the high and low ionization troughs for
the other outflow components, we show in Figure \ref{f7b} that the 
combination of the \siII\ composite template (described in section 3.3 
for component $\bf i$) and the \alii\ template (for all other components) 
can be used to recreate the doublet troughs of \mgii, 
\aliii, \siiv\ and \civ. Similar to Figure \ref{f8a}, we add two 
templates together in $\tau(v)$. We scale the entire blue template (all 
11 components) by one factor and scale the respective red template by 
2:1 in $\tau(v)$. This method gives the fewest possible constraints for 
the fit. We find that all 11 kinematic components are present in both 
low and high ionization troughs, and that there are no unexplained 
kinematic components in the higher ionization state lines, which is
indication that this is the same outflowing gas for both the high and 
low ionization troughs. We also note that these fits could be better 
if we scaled each individual component for the blue member and kept 
the 2:1 ratio to the red, as we did for the \aliii\ fit in Figure 
\ref{f8a}. 

\clearpage
\begin{figure}[!h]
  \centering \includegraphics[angle=0,width=0.7\textwidth]
  {Fig7.eps}\\
  \caption[]
  {\footnotesize The top left panel shows the \siII\ $\lambda$1527 
$\bf i$ component. The remaining panels show the agreement of the 
\siII\ $\lambda$1527 $\bf i$ component trough with the red 
doublet member of 5 other ions. The \siII\ $\lambda$1527 data has 
been converted to $\tau(v)$, where $\tau(v)$=-ln(I$(v)$), and
scaled by a single factor for each of the other lines in order to
produce the fits (red histograms) for these troughs (data shown in
black). Some discrepancy between the \siII\
$\lambda$1527 line and \aliii\ $\lambda$1863 occurs near 4000
km~s$^{-1}$, which is due to contamination from the blue $\bf k$
component. These agreements show that the ratio of column 
densities between each ion and \siII\ is constant across the 
profiles of the different troughs.}
  \label{f7a}
\end{figure}

\clearpage
\begin{figure}[!h]
  \centering \includegraphics[angle=90,width=0.9\textwidth]
  {Fig8.eps}\\
  \caption[]
  {\footnotesize Fits to the \aliii, \mgii, \civ\ and \siiv\ doublets with
the composite \siII\ template for component $\bf i$ and the \alii\
template for all other components. We add two templates in a similar
fashion as for Figure \ref{f8a}. These fits, however, are scaled by
one constant for the blue template and scaled by 2:1 for the red
template. We also include the \siII\ $\lambda$1527 resonance line 
and $\lambda$1533 excited line in the fit for \civ, which affect 
velocities greater than $\sim-$5500. These 4 fits clearly demonstrate 
that for each ion, all 11 components are present, and that no unexplained
components appear. We note that in the \civ\ fit there is evidence
for a component at $-$3600 km~s$^{-1}$ with a large optical depth
whereas the optical depth of this component \alii\ appears to be 
significantly lower, thus the template fit is poor. The fits would 
improve by scaling each component by a different factor in 
optical depth.}
  \label{f7b}
\end{figure}

\subsubsection{Measurements of the Other Components}

The other two components with a sufficient number of measurable 
absorption lines are the $\bf k$ and $\bf a$ components. However, we 
are unable to utilize methods 1 or 2 due to a lack of unblended \feii\ 
resonance lines. For component $\bf k$, only one \feii\ resonance line 
(\feii\ $\lambda$1608) is measurable and unblended. Thus, we measure 
the column densities based on a LOS covering factor of 1. We further 
confirm this assumption of a LOS covering factor of 1, as with the 
$\bf i$ component, by checking that the $\lambda$1608 line scales well 
to the unblended portion of \feii\ $\lambda$2383 according to oscillator 
strength. Component $\bf a$ has no measurable \feii\ resonance lines. 
However, according to the \aliii\ doublet (Figure \ref{f8a}), we find that 
a LOS covering of $\sim$1 holds for all components and we are able to 
resort to the AOD method for our measurements. The results for components 
$\bf k$ and $\bf a$ are shown in Tables~\ref{compk} and Table~\ref{compa} 
respectively.

Due to the lack of measurable, unblended troughs for components $\bf b$ 
through $\bf h$, we use the apparent optical depth method, and 
integrate the total column density across the combined blended troughs 
for components $\bf b$ through $\bf h$, $-$7150 to $-$4600 km s$^{-1}$ 
in velocity, for the \siiv, \civ, \mgii, and \aliii\ doublets as well as 
the resonance and excited lines of \cii\ ($\lambda$1335, $\lambda$1336) 
and \siII\ ($\lambda$1527, $\lambda$1533). We present these results in 
Table~\ref{compbh}.

\input{Table3}
\input{Table4}
\input{Table5}

\subsection{Estimates and Limits}

For situations where blending between components in doublets is 
prevalent (i.e. \civ, \siiv, \cii, and \cii*) or where the trough 
is heavily saturated (i.e., \civ), our primary method 
of column density extraction fails. Thus, we resort to other, less 
accurate, methods to estimate the column densities, 
which are important when constraining photoionization models. We 
develop three additional methods in order to estimate column 
densities in blended regions, which we explain here in order of 
decreasing accuracy.

In the first of our estimation methods (4), we opt to employ a 
template to map out approximate profiles for the troughs. We utilize
two templates for this process. The first template is a fit to the
\alii\ $\lambda$1671 line for all 11 components. However, due to 
moderate saturation in the core of the \alii\ $\bf i$ component, we 
create a composite template using the \siII\ resonance lines for 
the $\bf i$ component. 

To create this template, we use both the \siII\ $\lambda$1808 and
$\lambda$1527 lines. The $\lambda$1527 line is similar in shape to the
\alii\ $\lambda$1671 line, and while the core is moderately saturated,
it provides us with a good fit to the wings of the trough. In
contrast, the $\lambda$1808 line has a significantly weaker oscillator
strength and therefore the core of this trough is not saturated,
however the wings are buried in the noise. We therefore create a
composite template using the AOD column densities of the $\lambda$1527
for the wings (--3820 to --3990 \kms\ and --4390 to --4580 \kms), and
the AOD column densities of the $\lambda$1808 line for the core
(--4390 and -3990 \kms). We then convert the resultant \siII\ column
density profile to $\tau(v)$ template for the $\lambda$1527 line.

To measure column densities, we scale this composite $\tau(v)$
template to match the red wings of the \mgii, \siiv, and \civ\
doublets as well as \cii*, which are apparently free of blending. We
assume that the column density ratio is constant across the troughs,
which is supported by Figure \ref{f7a}, scale the composite template 
for the $\bf i$ component to match and then integrate the total column 
(assuming a
C$_{los}$$\approx$1) from the template. We refer to this method as the
``wing'' fitting method (method 4). The error estimation is provided
by using two $\tau$ scaling values, one underestimating and one
overestimating the noise level in the trough's wing.  We note that
these measurements use only one line, the red doublet member, which is
reflected in Tables~\ref{compi} through \ref{compbh}. To further test
the validity of this method, we used the composite template to fit the
wing of the \siII\ $\lambda$1527 line and we find that the template is
able to reproduce the column density we find in our power law fitting
of the $\lambda$1808 line to within 10\%. 

%\begin{figure}[!h]
%  \centering \includegraphics[angle=90,width=0.8\textwidth]
%  {Fig7.eps}\\
%  \caption[]
%  {\footnotesize
%Plot of the \cii\ $\lambda$1335 and \cii* $\lambda$1336 lines of the 
%$\bf k$ component with fits for the \cii\ and \cii* lines based on the 
%\alii\ template. The data are boxcar smoothed by 3 pixels. The blue 
%and green fits are for the \alii\ template scaled by 1.3 and 2.2 
%respectively in $\tau$ for \cii\, while the red and orange are for 
%$\tau$ scaled by 1.8 and 3.3 respectively for \cii*. We co-add the 
%average of these two fits in $\tau$ (in dashed light blue), which 
%appears to be an acceptable fit. We integrate the individual fits
%for the column densities (shown in Table 3).}
%  \label{f8}
%\end{figure}

The next method we designate as the ``tip'' fitting method, or method 
5, where we estimate the column densities in a similar 
way to method 4. For example, we estimate the column density of \oi\ 
$\lambda$1302 for the $\bf i$ component in the region containing 
blended lines from \siII\ $\lambda$1304 and \siII* $\lambda$1309. We 
find that the composite template fit for the $\bf i$ component agrees 
well with the deep trough at $\sim$3809 \AA\ in velocity space (shown
in online figure 1), which 
appears to be the tip of \oi\ absorption. Thus, we use the composite 
\siII\ template to approximate the minimum and maximum amount of column 
density that could come from \oi. Due to the uncertainty in continuum 
placement and possible saturation, we consider this method less accurate 
than method 4, which is reflected in the larger error bars.

Our last column density estimation method (the noise method or method 
6) defines upper limits on the column density of ions based on the 
statistical error of the data. Because the column density of \hei\ is 
important for photoionization models \citep[see][]
{2001ApJ...546..140A,2008arXiv0807.0230K}, we estimate an upper limit 
for the column density of the excited 2$^3$s level of \hei\ (\hei* 
hereafter) in component $\bf i$ for \hei* $\lambda$3189. To do this, 
we scale the \siII\ template for the $\bf i$ component and compare it 
to the region where the line would be detected. We vary the scaling 
to the noise level, find the largest possible optical depth that could 
be buried without detection and integrate across the template to determine 
the column density. We also perform this analysis for \mgi\ $\lambda$2853, 
\fei\ $\lambda$2484, and \ci\ $\lambda$1560; and quote the measured limits 
in Table~\ref{compi}. 

Component $\bf k$ presents its own problems. Unlike the $\bf i$ 
component, here we effectively measure column densities for \feii\ 
resonance and excited levels (E=0 cm$^{-1}$ to E=668 cm$^{-1}$), but 
we lack a \siII\ resonance line to provide a ratio to the \siII\ 
$\lambda$1309 excited line. Therefore, we apply method 5 with the 
\alii\ template to find limits on the \siII. Moreover, we use the 
``wing'' fitting method (method 4) with the same \alii\ template to 
estimate the column density for \cii\ and \cii* in component $\bf k$.

In component $\bf a$, the number of measurable lines is even fewer 
than for component $\bf k$. The only clean, unblended density 
diagnostic is \cii\ to \cii*. As the critical density for this ratio 
is low \citep[$\sim$10$^2$ cm$^{-3}$,][]{1992ApJS...80..425B,
1983JPHYSB..16..157},  it is important to find another density check. 
Thus, using the \alii\ template, we estimate an upper limit to 
the column density ratio of \siII* to \siII\ to be 0.49 for component 
$\bf a$. 

\subsection{Systematic Uncertainty}

We recognize 
that there exist systematic errors that could contribute further to
the uncertainty in our measurements. For example, our placement of the
continuum, defined in Section 2, could result in increased errors of
the \siII\ $\lambda$1808 and \siII* $\lambda$1817 column densities by
5\%. The amount of saturation in the core of \siiv\ is another
systematic error that could be a potential source of error in column
density, which at maximum, could lead to an error in ionization
parameter of 0.1 dex. Both of these are negligible compared to the
uncertainties due to the chemical abundance choice.



==> observation.tex <==
\section{Observations and Reduction}

During October of 2006, we obtained 8 echelle spectra, each with an 
exposure time of 2850 sec, of the object SDSS~J0318$-$0600 
\citep[z=1.967,][RA 03:18:56.7, Dec $-$06:00:37.4]{2007AJ....134..102S}
with the VLT. The observations were carried out by European Southern 
Observatory (ESO) staff and we present the observational parameters in 
Table~\ref{obs}. The spectra were taken using the UV-Visual Echelle Spectrograph 
(UVES) with a slit width of 1.0 arcsec, and a central wavelength position 
of 5800 and 3460 \AA\ for the red (Grating/Filter=CD1/HER5) and blue 
(Grating/Filter=CD3/SHP700) detectors respectively. A slit width of 1.0
arcsec gives a resolving power of $\sim$40000. The data were 
read out in a 2$\times$2 pixel-binned fashion, in high gain mode.

The data were extracted and calibrated using the standard UVES data 
reduction pipeline, based on ECHELLE routines, which is part of the 
reduction package MIDAS \citep{2000SPIE.4010..246B}. This calibration 
process can introduce quasi-periodic oscillations in amplitude in the
final spectral product \citep[see][on their analysis of QSO~2359-1241]
{2008ApJ...681..954A}, which can create up to 2-3\% systematic errors in 
continuum placement. The observations were corrected to heliocentric and 
subject to a cosmic ray removal procedure ($\sigma$ $>$ 3.5). We 
re-binned the data to 7.0 km s$^{-1}$, approximately one resolution
element, and normalized the spectrum using the methods described in 
\citet{2008ApJ...681..954A}.

\input{Table1} 

